A Step Towards Checking Security in IoT

The Internet of Things (IoT) is smartifying our everyday life. Our starting point is IoT-LySa, a calculus for describing IoT systems, and its static analysis, which will be presented at Coordination 2016. We extend the mentioned proposal in order to begin an investigation about security issues, in particular for the static verification of secrecy and some other security properties.

==> eptcsdata.tex <==
\providecommand{\firstpage}{128}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, S. Knight, and H. T. Vieira (Eds.):\\9th Interaction and Concurrency Experience (ICE 2016)\\
EPTCS 223, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.223.9}{10.4204/EPTCS.223.9}}
\pdfoutput=1

